Machine Learning Assessment: implications to cybersecurity

This chapter is dedicated to the assessment and performance estimation of machine learning (ML) algorithms, a topic that is equally important to the construction of these algorithms, in particular in the context of cyberphysical security design. The literature is full of nonparametric methods to estimate a statistic from just one available dataset through resampling techniques, e.g., jackknife, bootstrap and cross validation (CV). Special statistics of great interest are the error rate and the area under the ROC curve (AUC) of a classification rule. The importance of these resampling methods stems from the fact that they require no knowledge about the probability distribution of the data or the construction details of the ML algorithm. This chapter provides a concise review of this literature to establish a coherent theoretical framework for these methods that can estimate both the error rate (a one-sample statistic) and the AUC (a two-sample statistic). The resampling methods are usually computationally expensive, because they rely on repeating the training and testing of a ML algorithm after each resampling iteration. Therefore, the practical applicability of some of these methods may be limited to the traditional ML algorithms rather than the very computationally demanding approaches of the recent deep neural networks (DNN). In the field of cyberphysical security, many applications generate structured (tabular) data, which can be fed to all traditional ML approaches. This is in contrast to the DNN approaches, which favor unstructured data, e.g., images, text, voice, etc.; hence, the relevance of this chapter to this field.%

==> preamble-pgfplot.tex <==
\usepackage{pgf,pgfplots,pgfplotstable,tikz,tkz-fct}
\usepackage{tikz-timing}[2009/12/09]
\usepackage{float,fp}
\pgfplotsset{compat=1.11}
\pgfplotsset{width=7cm,compat=1.13}\usepgfplotslibrary{statistics}
\usetikzlibrary{calc,trees,positioning,arrows,chains,shapes.geometric,decorations.pathreplacing,decorations.pathmorphing,shapes,matrix,shapes.symbols,er,backgrounds,decorations.text,spy,automata}

\DeclareSymbolFont{letters}{OML}{cmm}{m}{it}

\DeclareMathOperator{\dist}{\mathbf{dist}}

\DeclareMathOperator{\dom}{\mathbf{dom}}

\DeclareMathOperator{\relint}{\mathbf{relint}}

\DeclareMathOperator{\aff}{\mathbf{aff}}

\DeclareMathOperator{\rank}{\mathbf{rank}}

\DeclareMathOperator{\bd}{\mathbf{bd}}

\DeclareMathOperator{\relbd}{\mathbf{relbd}}

\DeclareMathOperator{\conv}{\mathbf{conv}}

\DeclareMathOperator{\cl}{\mathbf{cl}}

\DeclareMathOperator{\R}{\mathbf{R}}

\DeclareMathOperator{\MSE}{MSE}

\DeclareMathOperator{\RMS}{RMS}

\DeclareMathOperator*{\E}{E}

\DeclareMathOperator*{\Var}{Var}

\DeclareMathOperator*{\Cov}{Cov}

\DeclareMathOperator*{\Corr}{Corr}

